Text-driven Affordance Learning from Egocentric Vision

Visual affordance learning is a key component for robots to understand how to interact with objects. Conventional approaches in this field rely on pre-defined objects and actions, falling short of capturing diverse interactions in realworld scenarios. The key idea of our approach is employing textual instruction, targeting various affordances for a wide range of objects. This approach covers both hand-object and tool-object interactions. We introduce text-driven affordance learning, aiming to learn contact points and manipulation trajectories from an egocentric view following textual instruction. In our task, contact points are represented as heatmaps, and the manipulation trajectory as sequences of coordinates that incorporate both linear and rotational movements for various manipulations. However, when we gather data for this task, manual annotations of these diverse interactions are costly. To this end, we propose a pseudo dataset creation pipeline and build a large pseudo-training dataset: TextAFF80K, consisting of over 80K instances of the contact points, trajectories, images, and text tuples. We extend existing referring expression comprehension models for our task, and experimental results show that our approach robustly handles multiple affordances, serving as a new standard for affordance learning in real-world scenarios.

==> tab/detailed_analysis.tex <==

\begin{table*}[t]
\centering
\caption{Detailed analysis of interaction regions prediction and trajectory estimation.}
\vskip 0.15in
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\scriptsize
\scalebox{0.91}{
\begin{tabular}{lclccccccccccccccccccccccccccccccc}
\toprule
                        & & & Desc. & \multicolumn{3}{c}{Heatmap $\uparrow$} & \multicolumn{2}{c}{Trajectory $\downarrow$} & \multicolumn{3}{c}{Heatmap $\uparrow$} & \multicolumn{2}{c}{Trajectory $\downarrow$} & \multicolumn{3}{c}{Heatmap $\uparrow$} & \multicolumn{2}{c}{Trajectory $\downarrow$} \\
                        \cmidrule(lr){5-7}\cmidrule(lr){8-9}\cmidrule(lr){10-12}\cmidrule(lr){13-14}
                        & & & & Sim & CC & AUC-J & ADE & DTW & Sim & CC & AUC-J & ADE & DTW & Sim & CC & AUC-J & ADE & DTW \\
\midrule
\rowcolor{Gray}
& & & & \multicolumn{5}{c}{\textit{Pick and Take}} & \multicolumn{5}{c}{\textit{Open}} & \multicolumn{5}{c}{\textit{Other verbs}} \\
\cmidrule(lr){5-9}\cmidrule(lr){10-14}\cmidrule(lr){15-19} 
\multirow{10}{*}{HO Int.} & \multirow{4.5}{*}{Seen}   
                        & VRB~\cite{vrb}      &  & \textbf{38.3} & \textbf{42.7} & 79.1 & \textbf{16.0} & \textbf{8.70} & 27.4 & 29.1 & 77.1 & 27.5 & 12.1\\
                        & & Lang-SAM & \checkmark & 35.7 & 40.8 & 68.3 & - & - & 28.1 & 32.6 & 71.4 & - & -\\
                        \cmidrule{3-13}
                        & & CLIPSeg~\cite{clipseg}  & \checkmark & 23.2 & 28.3 & 83.7 & 19.3 & 10.9 & 27.2 & 34.9 & \textbf{87.7} & 17.3 & 10.3 \\
                        & & MDETR~\cite{mdetr}  & \checkmark & 31.1 & 37.5 & \textbf{84.1} & 25.4 & 12.3 & \textbf{33.5} & \textbf{41.3} & 87.0 & \textbf{21.5} & \textbf{11.0} \\

\cmidrule{2-13}
& \multirow{4.5}{*}{Unseen} 
                        & VRB~\cite{vrb}      &  & \textbf{42.6} & \textbf{48.3} & 82.6 & \textbf{15.2} & \textbf{8.41} & 29.8 & 32.2 & 80.7 & 25.9 & 11.7\\
                        & & Lang-SAM & \checkmark & 39.9 & 46.1 & 74.7 & - & - & 29.9 & 35.1 & 78.9 & - & -\\
                        \cmidrule{3-13}
                        & & CLIPSeg~\cite{clipseg}  & \checkmark & 22.4 & 30.9 & \textbf{84.0} & 18.8 & 10.9 & 23.6 & 33.0 & 86.9 & 17.8 & 10.5 \\
                        & & MDETR~\cite{mdetr} & \checkmark & 26.3 & 31.5 & 82.3 & 24.2 & 12.0 & \textbf{32.5} & \textbf{40.0} & \textbf{88.3} & \textbf{22.8} & \textbf{11.5} \\
\midrule
\rowcolor{Gray}
& & & & \multicolumn{5}{c}{\textit{Cut}} & \multicolumn{5}{c}{\textit{Paint}} & \multicolumn{5}{c}{\textit{Other verbs}} \\
\cmidrule(lr){5-9}\cmidrule(lr){10-14}\cmidrule(lr){15-19} 
\multirow{10}{*}{HO Int.}   
                        & & VRB~\cite{vrb}      &  & \textbf{38.3} & \textbf{42.7} & 79.1 & \textbf{16.0} & \textbf{8.70} & 27.4 & 29.1 & 77.1 & 27.5 & 12.1\\
                        & & Lang-SAM & \checkmark & 35.7 & 40.8 & 68.3 & - & - & 28.1 & 32.6 & 71.4 & - & -\\
                        \cmidrule{3-13}
                        & & CLIPSeg~\cite{clipseg}  & \checkmark & 23.2 & 28.3 & 83.7 & 19.3 & 10.9 & 27.2 & 34.9 & \textbf{87.7} & 17.3 & 10.3 \\
                        & & MDETR~\cite{mdetr}  & \checkmark & 31.1 & 37.5 & \textbf{84.1} & 25.4 & 12.3 & \textbf{33.5} & \textbf{41.3} & 87.0 & \textbf{21.5} & \textbf{11.0} \\
\cmidrule{2-13}
& \multirow{4.5}{*}{Unseen} 
                        & VRB~\cite{vrb}      &  & \textbf{42.6} & \textbf{48.3} & 82.6 & \textbf{15.2} & \textbf{8.41} & 29.8 & 32.2 & 80.7 & 25.9 & 11.7\\
                        & & Lang-SAM & \checkmark & 39.9 & 46.1 & 74.7 & - & - & 29.9 & 35.1 & 78.9 & - & -\\
                        \cmidrule{3-13}
                        & & CLIPSeg~\cite{clipseg}  & \checkmark & 22.4 & 30.9 & \textbf{84.0} & 18.8 & 10.9 & 23.6 & 33.0 & 86.9 & 17.8 & 10.5 \\
                        & & MDETR~\cite{mdetr} & \checkmark & 26.3 & 31.5 & 82.3 & 24.2 & 12.0 & \textbf{32.5} & \textbf{40.0} & \textbf{88.3} & \textbf{22.8} & \textbf{11.5} \\

\bottomrule
\end{tabular}
}
\label{tab:more_detailed_analysis}
\end{table*}
% ``+dd.'' represents the use of deep decoder. 


==> tab/detailed_results_toi.tex <==

\begin{table*}[t]
\centering
\caption{Detailed analysis of interaction regions prediction and trajectory estimation in tool-object interactions.}
\vskip 0.15in
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\scriptsize
\scalebox{0.91}{
\begin{tabular}{lclccccccccccccccccccccccccccccccc}
\toprule
\rowcolor{Gray}
& & & & \multicolumn{5}{c}{\textit{Cut}} & \multicolumn{5}{c}{\textit{Close}} & \multicolumn{5}{c}{\textit{Other verbs}} \\
\cmidrule(lr){5-9}\cmidrule(lr){10-14}\cmidrule(lr){15-19} 
& & & Desc. & \multicolumn{3}{c}{Heatmap $\uparrow$} & \multicolumn{2}{c}{Trajectory $\downarrow$} & \multicolumn{3}{c}{Heatmap $\uparrow$} & \multicolumn{2}{c}{Trajectory $\downarrow$} & \multicolumn{3}{c}{Heatmap $\uparrow$} & \multicolumn{2}{c}{Trajectory $\downarrow$} \\
\cmidrule(lr){5-7}\cmidrule(lr){8-9}\cmidrule(lr){10-12}\cmidrule(lr){13-14}\cmidrule(lr){15-17}\cmidrule(lr){18-19}
& & & & Sim & CC & AUC-J & ADE & DTW & Sim & CC & AUC-J & ADE & DTW & Sim & CC & AUC-J & ADE & DTW \\
\midrule
& & VRB & & 9.3 & 11.8 & 68.5 & 36.2 & 14.6 & 37.4 & 39.8 & 94.8 & 15.7 & 8.9 & 26.0 & 27.5 & 73.5 & 28.5 & 12.4 \\
& & Lang-SAM & \checkmark & 12.0 & 9.2 & 59.9 & - & - & 51.7 & 61.7 & 97.3 & - & - & 21.7 & 24.6 & 62.3 & - & - \\
\cmidrule{2-19}
& & CLIPSeg & \checkmark & 31.9 & 48.4 & 95.0 & 14.8 & 8.8 & 35.8 & 60.5 & 96.2 & 18.5 & 11.1 & 26.5 & 38.6 & 89.5 & 17.8 & 10.3 \\
& & MDETR & \checkmark & \textbf{30.8} & \textbf{40.1} & \textbf{93.4} & 15.2 & 9.1 & 30.8 & 42.4 & 89.9 & 19.0 & 10.8 & \textbf{33.3} & \textbf{44.2} & \textbf{90.3} & \textbf{17.8} & \textbf{10.2} \\
                        
\bottomrule
\end{tabular}
}
\label{tab:more_detailed_analysis_toi}
\end{table*}
% ``+dd.'' represents the use of deep decoder. 

